Improved Robustness from Biologically Inspired Sparse Contrast Representations

Deep neural networks surpass humans on many vision benchmarks, yet remain far less robust to distribution shifts such as illumination and weather changes. Existing approaches address this challenge by additional training data, extensive augmentation, architectural modifications, or test-time adaptation. In this work, we explore a complementary direction: inspired by the human retina, we propose a fixed, model-agnostic preprocessing module that extracts signals that are more stable with respect to variations of illumination. Our method combines color remapping with local contrast extraction, producing sparse representations that emphasize structural features. We study its impact on semantic segmentation by training on Cityscapes and evaluating generalization under adverse conditions on Dark Zurich and ACDC. Our results show that the biologically inspired preprocessing preserves in-distribution performance while consistently improving robustness in challenging lighting scenarios, such as nighttime, where annotated training data are scarce. Moreover, the segmentation accuracy remains stable even when the contrast-based representation is sparsified by up to 70%. These gains suggest that rethinking the input representation itself can improve robustness while also opening opportunities for lower-latency, transmission-aware imaging sensors when sparsity can be exploited close to acquisition.

==> tex_for_figures/ablation_depth_parameter_search.tex <==
\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{figures/ablation_depth_paper.pdf}
  \caption{mIoU results for DeepLabv3+ (ResNet-18) trained on Cityscapes and evaluated on Cityscapes, Dark Zurich, and ACDC night datasets. Results are reported for each depth value from 0 to 10. Balancing overall robustness (Dark Zurich and ACDC Night) and accuracy on i.i.d.~data (Cityscapes), we observe that $\mathrm{d}=5$ is the best candidate across preprocessing variants. For other metrics please refer to the appendix.}
  \label{fig:Validation results - Depth Parameter Search}
  \vspace{-0.5em}
\end{figure*}
